Hagedorn String Thermodynamics in Curved Spacetimes and near Black Hole Horizons

This thesis concerns the study of high-temperature string theory on curved backgrounds, generalizing the notions of Hagedorn temperature and thermal scalar to general backgrounds. Chapter 2 contains a review on string thermodynamics in flat space, setting the stage. Chapters 3 and 4 contain the detailed study of the random walk picture in a general curved background. Chapters 5 and 6 then apply this to Rindler space, the near-horizon approximation of a generic (uncharged) black hole. Chapters 7 and 8 contain a study of the AdS3 and BTZ WZW models where we study the thermal spectrum and the resulting random walk picture that emerges. Chapters 9 and 10 attempt to draw general conclusions from the study of the two specific examples earlier: we draw lessons on string thermodynamics in general and on (perturbative) string thermodynamics around black hole horizons. For the latter, we point out a possible link to the firewall paradox. Finally, chapter 11 contains a detailed discussion on the near-Hagedorn (and high-energy) stress tensor in a generic spacetime, the results of which are applied to provide a description of the Bekenstein-Hawking entropy in terms of long string equilibration.

==> Preface.tex <==
\thispagestyle{empty}

%\centerline{\LARGE \textsf{Preface}}
\centerline{\LARGE Preface}
\vspace{1.5cm}
\noindent This PhD work could not have been completed without the support and advice from many friends, colleagues and relatives, so some words of thanks are in order. \\

\noindent Firstly, I would like to thank Henri for giving me the opportunity the past four years to study aspects of string theory and for allowing me the freedom to pursue whatever I found interesting. In particular, I clearly remember the lessons on QFT as a student and the level of enthousiasm of Henri while teaching this course. This really motivated me into a PhD in high energy theoretical physics. \\
Next I thank Valya and Henri for the many discussions on black holes, strings and thermal physics. Also many thanks for showing me how to think in physics, which questions to pursue and the general support during the past four years of fruitful collaboration. \\

\noindent I also owe a great deal of gratitude to David, for the interesting collaboration the last two years but also (and mainly) for the many discussions during lunch. These discussions taught me a lot on theoretical physics and at the same time provided an ideal opportunity to test ideas in front of a critical audience! \\

\noindent I would also like to thank several colleagues: Hans (for amusing discussions about how our long strings are related to vortices in the heart), Boye, Karel and Dirk. And also my office colleagues (in order of appearance): Fr\'ed\'eric, Vid, Nele, Benjamin, Igor and Diego. I thank you for the many joyful conversations and discussions (both on- and off-topic). \\
\noindent Researchwise, I would like to thank Ben Craps, Oleg Evnin, Amit Giveon, Nissan Itzhaki, Hampus Linander, Lihui Liu, Shiraz Minwalla, Blagoje Oblak, Jo\~{a}o Penedones, Waldemar Schulgin, Chung-I Tan, Joris Vanhoof, Herman Verlinde and Frank Verstraete for interesting discussions on the topics presented here at various stages during the completion of this work. \\

\noindent Financially, I am grateful to the UGent Special Research Fund. \\

\noindent On a recreational level, I thank the documentary series `Cosmos' and the movie `Interstellar' for providing a `catalyst' for discussions on black holes with both family and friends and for bringing these exciting topics to a wider audience. \\

\noindent Finally, I thank my friends, my parents, my grandparents and my sister for the support during the years and for listening to / enduring all of my physics monologues, wanted or not! \\

\vspace{0.5cm}
\textit{Thomas Mertens, \hspace{0.5cm}March 2015, \hspace{0.5cm}Ghent}

